Serving Deep Learning Model in Relational Databases

Serving deep learning (DL) models on relational data has become a critical requirement across diverse commercial and scientific domains, sparking growing interest recently. In this visionary paper, we embark on a comprehensive exploration of representative architectures to address the requirement. We highlight three pivotal paradigms: The state-of-the-art DL-centric architecture offloads DL computations to dedicated DL frameworks. The potential UDF-centric architecture encapsulates one or more tensor computations into User Defined Functions (UDFs) within the relational database management system (RDBMS). The potential relation-centric architecture aims to represent a large-scale tensor computation through relational operators. While each of these architectures demonstrates promise in specific use scenarios, we identify urgent requirements for seamless integration of these architectures and the middle ground in-between these architectures. We delve into the gaps that impede the integration and explore innovative strategies to close them. We present a pathway to establish a novel RDBMS for enabling a broad class of data-intensive DL inference applications.

==> background.tex <==
\section{Background and Related Works}
\label{sec:background}

In this section, we review the existing benchmarks for deep learning frameworks and decision support workloads in RDBMS. Then, we describe how these works can be leveraged to design meaningful benchmark for the proposed unique comparison of various  representations of deep learning inference workloads in RDBMS.

\subsection{Benchmarks for Deep Learning Inferences} The best-known benchmark for deep learning infercence workloads is the MLPerf inference benchmark~\cite{mattson2019mlperf, reddi2020mlperf}, which is built on top of the
DawnBench~\cite{coleman2017dawnbench}. The latest version of MLPerf inference benchmark~\cite{MLCommons} mainly includes following workloads for the data center and the edge environments: (1) Image classification using the Resnet50 model on the ImageNet dataset; (2) Object detection using the ResNet34 model and SSD-MobileNets-v1 model on the COCO dataset; (3) Medical image segmentation using the 3D UNET model on the Bras 2019 dataset; (4) Speech-to-text using the RNNT model on the Librispeech dataset; (5) Language processing using the BERT-large model on the SQuAD dataset; (6) Recommendation using the DLRM model on top of the 1TB Click logs; among other benchmark workloads. The MLPerf Inference benchmark consists of four evaluation scenarios: single-stream, multistream, server, and offline. It also defines the accuracy target besides the latency target for each model and scenario. 

Fathom~\cite{adolf2016fathom} is a set of reference implementations of a broad class of deep learning models including (1) Sequence-to-sequence translation using a multi-layer pipeline of LSTM model; (2) Natural language reasoning problem using Facebook AI's memnet architecture; (3) Speech recognition using Baidu's Deep Speech model, which is five fully-connected layers of 2048 neurons each with one bidirectional recurrent layer; (4) Variational autoencoder for feature learning; (5) Image classification using the residual network on the ImageNet dataset; (6)  VGG-19 on the ImageNet dataset; (7) AlexNet on the ImageNet dataset; and (8) Atari-playing using deep reinforcement learning from DeepMind.

All of DawnBench Inference~\cite{coleman2017dawnbench}, MLPerf Inference~\cite{reddi2020mlperf}, and Fathom Inference~\cite{adolf2016fathom}, chose representative and widely-accessible deep learning models for realistic evaluation. However, they did not consider the integration with RDBMS. Therefore, these benchmark suites do not represent popular deep learning inference workloads in RDBMS and do not address the relational queries that are nested with the model inferences.

Besides the aforementioned benchmarks that target at evaluating an end-to-end model inference process, DeepBench~\cite{deepBench} aims at benchmarking a limited set of kernel-level operations that are important to deep learning and widely used in various deep neural networks. It consists of the training benchmark and the inference benchmark. The inference benchmark  mainly consider three types of operations: the dense/sparse matrix multiplication, convolutions, and the recurrent layers such as long short-term memory (LSTM) and gated recurrent unit (GRU). While it is relatively easier to implement DeepBench in the RDBMS environment, it cannot address the complexity of full models and an end-to-end inference-query scenario.

In addition, AI benchmark~\cite{ignatov2019ai} and EEMBC MLMark~\cite{torelli2019measuring} are both mobile-inference benchmark suites and they focus on the latency of image processing models on various smart phone or embedded devices. 

The TPCx-AI benchmark~\cite{council2021tpc} emulates real world AI scenarios and data science use cases. Unlike most
other AI benchmarks, the TPCx-AI uses a diverse dataset and is able to scale across a wide range of scale factors. In addition, the TPCx-AI benchmark has a focus on traditional ML. Among the ten use cases defined in TPCx-AI, only two use cases adopt deep learning models: DeepSpeech for the use case 2 of  customer conversation transcription; and RNN for the use case 6 of price prediction. Other eight use cases all adopt traditional ML techniques such as k-means for customer segmentation,  Auto-Regressive Integrated Moving Average (ARIMA) for sales forecasting, Naive Bayes for spam detection, Support-Vector machines (SVM) for hardware failure detection, matrix factorization based on Alternating
Least Squares (ALS) for product rating, logistic regression for facial recognition and fraud detection, etc. For all use cases, the features are extracted from the same database that consist of $14$ relations. Each use case has also defined an end-to-end data science process including the data cleaning, preprocessing, labeling, model training, validation, deployment, and serving.



\subsection{Benchmarks of Relational Queries} 
There are several benchmarks widely used as industrial standard benchmarks for commercial database systems.

The TPC-H benchmark~\cite{poess2000new} is a decision support benchmark. It consists of eight base tables that model an e-commerce company. The TPC-H benchmark generates the database scaling from $1$GB to $100$TB. It defines $22$ parameterized adhoc query templates that answers various business questions. This benchmark is widely used in academia and industry.

The TPC-DS benchmark~\cite{nambiar2006making} is designed to address the shortcomings of TPC-H such as the unrealistic data distribution. It models a retail company
that sells goods through the three distribution channels: store, catalog
and Internet (web). An inventory fact table is shared between the
catalog and the Web channels. The
TPC-DS benchmark generates the database, which also scales from
$1$GB to $100$TB, following real-world data distribution. The TPC-DS benchmark defines $99$ parameterized
query templates to model the reporting tasks, ad hoc decision support tasks,etc. 

TPC-C is an On-Line Transaction Processing Benchmark~\cite{council1996tpc}, which portrays the activity of a wholesale supplier and any industry that must
manage, sell, or distribute a product or service (e.g., car rental, food distribution, parts supplier, etc.). The supported transactions include the new-order transaction, the payment transaction, the order-status transaction, the delivery transaction, the stock-level transaction, etc.

Other popular benchmarks include but not limited to JCC-H~\cite{boncz2017jcc}, which introduces join-crossing-correlations
and skews into TPC-H; The CH Benchmark~\cite{cole2011mixed} that combines TPC-H
and TPC-C to evaluate database systems on hybrid transaction and
analytical (HTAP) workloads; and the DSB benchmark~\cite{ding2021dsb}, which is designed for evaluating both workload-driven and traditional database
systems on modern decision support workloads. 




==> codegen.tex <==
\section{Code Generation}
\label{sec:codegen}

The IR, after optimization, will be further split into pipeline stages. A pipeline stage consists of a series of operators. The first operator scans materialized data (e.g., a cutomer dataset, an intermediate dataset, or a shuffled dataset). The last operator materialize data to file, or for shuffling. All intermediate operators will not materialize data. The next goal is to generate highly efficient data-centric code~\cite{neumann2021evolution} for each pipeline stage. The generated code should be vectorized, memory-efficient, and fully pipelined (i.e., operators are fused). In addition, for those operators that may benefit from hardware acceleration, we also want to apply hardware acceleration by generating GPU code. We identified the challenges as follows:

\vspace{5pt}
\noindent
\textbf{Challenge 8.} How to partition the processing for C++ and MLIR/LLVM code generation respectively?

It is hard to automatically generate code for the entire query processing process. On one hand, a significant portion of the processing logic, e.g., executing a pipeline stage (i.e.,), shuffling \texttt{<key, value>} pairs, is query independent, and can be pre-compiled. Compiling these logic at runtime for each query requires significant amount of query compilation overheads, which should be avoided. On the other hand, it could be complicated to automatically glue UDFs together for pipelining, parallelization, etc.

One approach is to implement a parallelized and pipelined execution framework in C++, and use the MLIR/LLVM framework to generate the code for operators that are customized by UDFs and user defined types (UDTs). 

\vspace{5pt}
\noindent
\textbf{Challenge 9.} How to partition the logic for executing on CPU and GPU respectively?

GPU is not only widely used to accelerate linear algebra computations, but also applied to accelerate relational processing. Recently, there are abundant existing works, such as Crystal~\cite{shanbhag2020study}, HeavyDB~\cite{heavydb}, BlazingSQL~\cite{blazingsql}, PG-Storm~\cite{pg-storm}, and TQP~\cite{he2022query}, accelerating relational algebra operations using GPU. 
However, recent studies~\cite{cao2023revisiting, guan2023comparison} show that if the operation is insufficient to fully utilize the GPU resource, the transfer of data between CPU and GPU could become the bottleneck. On one side, a single inference query that involves small amount of data and small model may not benefit from GPU acceleration. On the other side, we may consider running multiple inference queries that involve small data and small model on the GPU device concurrently. Recent advances in multi-instance GPU~\cite{li2022characterizing} provides a convenient interface for using GPU to accelerate multi-tenant inference query execution.

In addition, many queries that involve non-numerical data, e.g., string values, require pre-processing to convert such data to numerical data through encoding to utilize GPU~\cite{cao2023revisiting, he2022query}, which incurs non-trivial overheads. This mean the query optimization process should take data/model sizes, data types, and query concurrency into consideration when selecting operations to run in GPU.


\vspace{5pt}
\noindent
\textbf{Challenge 10.} How to schedule computations to overlap the CPU computation, I/O operations (e.g., shuffling, disk reading/writing), and GPU computation?

Because each pipeline stage may be fully executed in CPU, fully executed in GPU, or have portions of operators executed in CPU and the rest of operators executed in GPU, it is important to carefully schedule the pipeline stages in order to fully utilize the CPU and GPU resources and overlap I/O operations and computations. 

A promising approach is to use the producer-transfer-consumer (PTC) model~\cite{shi2014mrtuner} to model the consecutive CPU and GPU operations within one pipeline stage, and to model two consecutive pipeline stages.




==> compiler.tex <==
\section{Unified Compilation Framework}
\label{sec:compilation}
\subsection{Intermediate Representation}

In this section, we focus on the below challenge.

\vspace{5pt}
\noindent
\textbf{Challenge 1.}  How to design the IR to meet the following requirements: (1) Represent both relational query processing and DNN model processing; (2) Facilitate dynamic representation of some kernels in a DNN model as UDFs, and some kernels as relational operators; (3) Facilitate more techniques that facilitate SQL query processing and DNN model inferences.

To explore the opportunities to address this challenge, we first review existing IRs.

\noindent
\textbf{Deep learning IRs.} To represent the DNN processing, it is straightforward to leverage graph IRs that are widely used in TensorFlow/XLA~\cite{olston2017tensorflow}, Pytorch 2.0/TorchDynamo/TorchInductor~\cite{wu2023pytorch}. In such graph IR, each node represents a deep learning kernel (e.g., convolution, matrix multiplication), and each edge represents a tensor that is created from the source node and is fed to the target node. Such graph IR can be used to represent a broad class of DL models. In addition, for new custom kernels that are not supported by the above-mentioned graph IR, they can be described in Tensor Expression Language~\cite{chen2018tvm} as adopted in TVM. Such tensor expressions will be used for automatic search for optimal implementation and code generation for new hardware. Moreover, the recent development and open source of the Multi-Level Intermediate Representation (MLIR)~\cite{mlir, lattner2021mlir} by Google and LLVM integrate multiple levels of IR dialects for machine learning processing. 

\noindent
\textbf{Relational and Dataflow IRs.} Relational algebra is used to represent relational processing. In relational algebra, each node represents a relational operator (e.g., \texttt{join}, \texttt{aggregate}, \texttt{selection}, \texttt{projection}). It is often extended to nest UDFs to support user-defined analytics over schema-flexible datasets. UDFs can be represented in a lower-level IR such as WeldIR~\cite{palkar2017weld} to facilitate cross-library optimization, Lachesis~\cite{DBLP:journals/pvldb/ZouDBIYJJ21} to facilitate data reorganization, or an even lower-level IR such as LLVM IR~\cite{crotty2015architecture} for code generation, among other UDF IRs such as Froid~\cite{ramachandra2017froid}, Emma/Lara~\cite{alexandrov2015implicit, kunft2019intermediate}. Daphne IR ~\cite{damme2022daphne} and LingoDB~\cite{jungmair2022designing} both implement the dataflow IR and relational algebra IR as dialects of MLIR so that the relational processing and deep learning processing can be integrated into the same MLIR compilation framework~\cite{mlir, lattner2021mlir}. Tensor Relational Algebra~\cite{yuan2020tensor} is an example of this type of IR, where all linear algebra computations will be translated to relational operators. As we mentioned in Sec.~\ref{sec:performance}, although it can scale better and easier to large-scale models, it will lead to sub-optimal performance for small-scale models.

\vspace{5pt}
\noindent
We discuss two options, which represent different opportunities:

\noindent
\textbf{Option 1: Multi-level IR}.  Shaikhha et al~\cite{shaikhha2016architect} proposed to have multiple levels of intermediate representations to improve the flexibility of the query compilation process. However, it doesn't consider the extension to AI/ML inference queries. Recently, LingoDB~\cite{jungmair2022designing} and Daphne IR~\cite{damme2022daphne} provide an MLIR dialect for relational processing, which can serve as a nice foundation for integrating with existing dialects for AI/ML computations developed by the MLIR community, including high-dimensional tensor abstraction dialects such as Tensor, Arith, Linalg, and high-dimensional vector abstraction such as Vector and SCF, to facilitate cross-optimizations within the MLIR framework. However, they haven't found a way to fully integrate MLIR and relational database runtime. For example, LingoDB~\cite{jungmair2022designing} doesn't support complicated data processing such as parallel query execution, caching, and spilling data to disk. 
Integrating database query optimization, query scheduling, and buffer management with MLIR could be very challenging~\cite{neumann2011efficiently, neumann2021evolution}, but worthy of exploration. 

\vspace{3pt}
\noindent
\textbf{Option 2: Adaptive in-Database IR}. An alternative is to implement an adaptive IR within RDBMS, where each node is either a traditional relational operator or a model UDF operator. A model UDF operator corresponds to a DL model inference computation. The model UDF is further expressed as a subgraph, where each node represents a linear algebra operator such as matrix multiply, matrix add, relu, softmax, conv2d, etc. Each such linear algebra operator can be flexibly converted into relational algebra operators. For example, a matrix multiply can be replaced by a join followed by an aggregation as aforementioned, if such conversion brings performance benefits (e.g., break-down a large-scale matrix multiplication to relational processing over two large collections of matrix blocks to fit the multiplication into memory). The idea shares some similarities with the Raven IR~\cite{park2022end} which provides a hybrid IR where each operator is either a relational operator or an atomic DL operator. The difference is in the nativeness to RDBMS and the adaptivity/flexibility to encapsulate multiple DL operators into a coarse-grained UDF and/or convert one more more DL operators into relational operators.












\subsection{Query Optimization}
\label{sec:optimization}

Distinguished from existing cost-based query optimizers, the inference query optimizer is faced with new challenges:

\vspace{5pt}
\noindent
\textbf{Challenge 2.}  Existing query optimizers and query graph transformation rules may not be able to capture a lot of co-optimization opportunities for deep learning. For example, one common optimization is to compress the model to sacrifice some accuracy in order to gain faster inference time~\cite{kang2018blazeit, kang2017noscope}. In addition, the weight matrix of some neural networks e.g., fully connected layers, can be partitioned into multiple sub-matrices by features. Each of the sub-matrices has an option to be pushed down to reduce the amount of intermediate data that needs to be joined, similar to vertical federated learning~\cite{le2021fedxgboost, chen2021secureboost+, chen2021fed}. Furthermore, if translated to relational computations, how we block the tensor to form a collection of tensor blocks (i.e., tensor relation) will significantly impact the tensor computations~\cite{luo2021automatic}. These new requirements are all beyond the scope of the existing query optimization process.

To address this challenge, opportunities may exist in leveraging the recent progresses made in AI/ML community about AutoML and deep learning compilation. For example, existing Neural Architecture Search (NAS) frameworks such as Zero shot NAS~\cite{lin2021zen}, Efficient NAS based on parameter sharing (ENAS)~\cite{pham2018efficient}, etc., automatically search for model architectures that balance accuracy and model sizes or computational complexities. Deep learning compilers, such as AutoTVM~\cite{chen2018learning} and flexible storage optimization~\cite{schleich2023optimizing},  automatically search for optimal tiling and computation patterns. 

\vspace{5pt}
\noindent
\textbf{Challenge 3.}  For complicated inference queries that involve large-scale models, such as large language models, the search space for the co-optimization techniques could be significantly larger than traditional SQL queries.


\noindent
\textbf{Challenge 4.} Although many popular model architectures are deterministic, there emerge dynamic models~\cite{zheng2022dietcode}, of which the shapes of tensors are unknown until runtime, which poses new cardinality estimation challenges.


\noindent
\textbf{Challenge 5.} The optimization and compilation for each ad hoc inference query could be expensive. How to alleviate the costs for a group of queries that involve the inferences using the same model?


To address these challenges, 
 in addition to standard techniques such as learning-based optimization~\cite{kim2022learned},  Bayesian optimization~\cite{frazier2018tutorial}, and query graph partitioning~\cite{jankov12declarative}, we consider ahead-of-time (AoT) compilation~\cite{zhang2021adaptive, lee2018pretzel}. For example, DietCode~\cite{zheng2022dietcode} optimizes dynamic tensor shapes for a dynamic model by generating multiple execution plans at compilation time and selecting the best plan at runtime.  
Compared to just-in-time (JIT) compilation, AoT compilation could save a lot of runtime optimization and compilation overheads. 
However, it is difficult to predict runtime ad hoc behaviors based on static analysis, such as which SQL predicates will be nested with the model inference queries, and which batch size could be optimal in meeting users' service level agreement (SLA). For example, credit card fraud detection queries usually involve the same model, except that the query structure, query parameters, and batch size will be dynamic at runtime. One idea is that we may cluster the possible inference queries that involve the inferences using the same model into several categories, and compile models for each category. Then, at runtime, the system selects one pre-compiled representation of the models and compiles the rest of the queries, rather than compiling the entire query from scratch. This will alleviate the compilation overheads for a broad class of inference queries that involve complicated/dynamic models and the frequent execution of queries that involve similar models. 



\subsection{Code Generation and Vectorization}

There has been a long-standing debate in the database community about whether to use code generation (i.e., compilation)~\cite{neumann2011efficiently, neumann2021evolution, shaikhha2018building} or vectorization~\cite{boncz2005monetdb, padmanabhan2001block, zukowski2009balancing} for query processing. According to a comparison study~\cite{kersten2018everything}, the performance of vectorized and 
compiled query execution is quite similar for OLAP workloads. Recently, because vectorized query processing can avoid the lengthy compilation process for complicated queries, many systems such as Photon from Azure Databrick~\cite{behm2022photon} and Velox from Meta~\cite{pedreira2022velox} mostly adopted vectorized query processing, or a hybrid approach, e.g., only relying on templated meta-programming for code generation~\cite{zou2018plinycompute}. 

Interestingly, there have been similar debates in the ML community. One option corresponds to the graph-based IR, as adopted by almost all ML frameworks such as TensorFlow, Pytorch 2.0. It is to lower each node in the graph (i.e., a kernel) to a call of APIs from existing libraries, such as Intel MKL~\cite{wang2014intel}, CuDNN~\cite{cudnn}, CuBLAS~\cite{cublas}, IBM zDNN~\cite{zdnn}. This approach cannot generalize to new kernels and new hardware, which do not have reliable and high-performance library implementations. Another option is based on tensor expression language, and the optimizer automatically searches for a tensor computation algorithm and generates code for the target hardware, which is adopted by TVM~\cite{chen2018tvm}, Halide~\cite{ragan2013halide}, Tensor Comprehension~\cite{vasilache2018tensor}, and so on. This approach may suffer from the lengthy compilation time for complex models (e.g., large language models), due to the huge search space.   

\vspace{5pt}
Naturally, a new challenge for inference query compilation is:


\noindent
\textbf{Challenge 6.} How shall we combine a compilation (i.e., code generation) approach and an approach that mainly leverages fully optimized pre-built vectorized relational operators, vectorized data processing functions, and known linear algebra computations? 

A potential solution is to lower those known relational operators and linear algebra operators to existing vectorized data processing operators and fully optimized tensor library functions, and at the same time, to use a compilation approach to generate code for unknown UDFs and ML kernels. 


==> experiments.tex <==










\eat{
 

}






\eat{
\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:velox-latency} {\small \color{black} End-to-End Latency Comparison on Velox for the MNIST Workloads. Batch size are tuned for TensorFlow (TF) and Pytorch (unit: seconds)}}
\begin{tabular}{|r|r|r|r|} \hline
Dataset size & Velox-UDF & Decoupled-TF & Decoupled-PyTorch \\\hline \hline
$1000$&$\textbf{0.04}$&$0.5$&$0.16$\\
$10000$&$\textbf{0.19}$&$1.1$&$0.52$\\
$60000$&$\textbf{0.80}$&$4.36$&$2.45$\\
\hline

\hline
\end{tabular}
\end{table}
}





==> extension.tex <==
\section{Extend DB Functionalities to DL Inferences}
\label{sec:functionality}
Among many DB functionalities, we pick the fine-grained access control over logical views as an example.  Given a query, the database will automatically check whether the query issuer has the corresponding privileges to access the data involved in the query. In addition, recent research provides differential privacy (DP) guarantees to SQL queries~\cite{johnson2018towards} and can automatically add noises to the query results to meet a privacy budget. %
The Relation-Centric approach naturally benefits from RDBMS' automatic access control advantages (as it treats each weight tensor as a regular relation, allowing users to define access control rules). However, in the DL-Centric approach, the models are stored in DL formats like HuggingFace and ONNX model formats, which are not directly interpretable by the RDBMS storage and catalog manager, making fine-grained access control challenging. Similarly, for the UDF-Centric approach, weight tensors are local variables of the UDF function and are opaque to the RDBMS. Consequently, neither of these approaches can fully leverage these functionalities, requiring developers to implement security and privacy protection at the application level. This increase in development costs slows down the time-to-market.

\vspace{5pt}
\noindent
\textbf{Challenge 1.} How to extend RDBMS security and privacy functionalities to the DL-Centric and UDF-Centric approaches, and work with DL mechanisms that protect models from the stealing/extraction attacks~\cite{tramer2016stealing, tian2021probabilistic} and membership inference attacks~\cite{shokri2017membership, abadi2016deep}?

First, the RDBMS should manage DL models as relations in storage and catalog  for the DL-Centric and UDF-Centric approaches,  enabling the application of the security and privacy mechanisms in RDBMS. %
Second, the storage of a DL model should expose sufficient information to the RDBMS. For example, if the model has been trained with differential privacy (e.g., using DP-SGD~\cite{abadi2016deep}), it should notify RDBMS about the DP parameters, such as the privacy budget.  Then, RDBMS is able to account privacy budget for inference queries that rely on the model. %
 Third,  data and models' security and privacy levels need to be consistently designed for use cases. For example,  if the model has been trained using a relation managed by the RDBMS, the RDBMS should associate the model with the relation (i.e., the training dataset). Then, the access control policies defined over the relation can be passed to the model. Moreover, the DB privileges may be extended to consider Train/Predict with a specific privacy budget in addition to Read/Write.


==> interface.tex <==
\section{User Interface}

\noindent
\textbf{Challenge 1.} The new query compilation framework should support the loading of DNN models that are trained using popular frameworks such as Scikit-Learn, TensorFlow, Pytorch, MXNet. The opportunity is that there exist standard model formats such as ONNX~\cite{onnx, bai2019onnx}, which supports transforming from models trained by most of these popular AI/ML frameworks. Therefore, we can start by supporting the loading of ONNX models to RDBMS and introducing new commands such as "CREATE MODEL" and "LOAD MODEL". The first command specifies the model name and model metadata, while the second command specifies the path to the ONNX model to be loaded into the RDBMS. 


\vspace{5pt}
\noindent
\textbf{Challenge 2.} Unlike existing model serving frameworks that use RESTful APIs or Python APIs, the inference of the model should be easily represented as a query over datasets that are managed by the RDBMS. Most importantly, through the new interface, we should be able to integrate the inferences with other existing DB logics. The users should be able to integrate the model inferences and the data preprocessing (e.g., featurization, curation, normalization, imputation, etc.) in one query task in the analytics database to facilitate co-optimization, as illustrated in Listing~\ref{lst:queries}.

\begin{lstlisting}[
        caption={Example inference queries},label={lst:queries},
           language=SQL,
           showspaces=false,
           basicstyle=\ttfamily\small,
           numbers=left,
           numberstyle=\tiny,
           commentstyle=\color{gray},
           breaklines=true
        ]
SELECT count(*) FROM transactions WHERE fraud_dnn.predict(*) = True GROUP BY created_on;
SELECT recommend_dnn.predict(*) FROM transactions, customers WHERE  transactions.customer_id = customers.id AND transactions.transaction_id = $transaction_id
\end{lstlisting}

Besides, the users should be able to incorporate inference queries into transactions as shown in Listing~\ref{lst:transaction}.

\begin{lstlisting}[
        caption={An example transaction mixing model inferences},label={lst:transaction},
           language=SQL,
           showspaces=false,
           basicstyle=\ttfamily\small,
           numbers=left,
           numberstyle=\tiny,
           commentstyle=\color{gray},
           breaklines=true
        ]
BEGIN;
INSERT INTO transactions VALUES ($transaction_id, $processor_id, $processor_name, $transaction_type, $document_no, $document_type, $document_group, $customer_id, $currency_id, $account_no, $amount, $auth_code, $card_type, $created_on);
UPDATE transaction_fraud_detection SET fraud = (SELECT (fraud_dnn.predict(*))FROM transactions WHERE transaction_id=$transaction_id) WHERE transaction_id=$transaction_id;
UPDATE accounts SET balance = balance - $amount WHERE account_no = $account_no_to_debit AND (SELECT fraud FROM transaction_fraud_detection WHERE transaction_id=$transaction_id)=False;
UPDATE accounts SET balance = balance + $amount WHERE account_no = $account_no_to_credit WHERE account_no = $account_no_to_debit AND (SELECT fraud FROM transaction_fraud_detection WHERE transaction_id=$transaction_id)=False;
COMMIT;

\end{lstlisting}







==> ir.tex <==
\section{Intermediate Representation (IR)}

There exist many types of IRs that are related with our vision.

To represent the DNN processing, we can leverage a graph IR that is widely used in TensorFlow, MXNet, and Pytorch Glow. In the graph IR, each node represents a deep learning kernel (e.g., convolution, matrix multiplication, etc.), and each edge represents a tensor that is created from the source node and is fed to the target node. Such graph IR can be used to represent a broad class DNN models, but it cannot represent relational processing and UDFs. 

Relational algebra are used to represent relational processing in RDBMS. In relational algebra, each node represents a relational operator (e.g., join, aggregation, selection, projection). Then it is extended to nested relational algebra to support UDFs and to dataflow graph to support user defined analytics over schema-flexible datasets. Recently, we extended it to Tensor Relational Algebra (TRA) to customize relational operators using various kernels (as UDFs) that operates over tensor blocks.

Further more, RDBMS user defined functions or library functions can be represented in a lower-level IR such as WeldIR and Lachesis, or an even lower-level IR such as LLVM IR.

However, none of these IRs can resolve the two bottleneck problems of our vision: 

\vspace{5pt}
\noindent
\textbf{Challenge 3.}  How to design the IR to integrate and facilitate co-optimization of relational query processing and DNN model processing?

\noindent
\textbf{Challenge 4.}  How to design the IR to facilitate dynamic representation of some layers in a DNN model as UDFs, and some layers as relational operators?

\vspace{5pt}
While both problems are challenging, the recent development and open source of the Multi-Level Intermediate Representation (MLIR) library by Google and LLVM provides an opportunity to address these problems. One approach is to implement two levels of IRs as MLIR dialects. 

The first MLIR dialect is an upper-level IR based on nested relational algebra. Each operator represents an atomic relational operator including but not limited to the following:

\noindent
(1) \texttt{applyFunc}, which is to apply a UDF that is defined in user code (e.g., an .so library provided by the user).

\noindent
(2) \texttt{filter}, which is to filter a vector of objects based on a vector of boolean values, where each boolean value corresponds to one object. 

\noindent
(3) \texttt{hash}, which is to convert a vector of objects into a vector of hash values.

\noindent
(4) \texttt{equiJoin}, which is to join two vectors of <key, value> pairs based on the equality of the keys.

\noindent
(5) \texttt{groupBy}, which is to split a vector of <key, value> pairs into multiple groups by keys, so that each group corresponds to one key, and contains a list of values that have been paired with the key. 

The second MLIR dialect is a lower-level IR based on the ML graph intermediate representation. Each operator represents an linear algebra kernel (or tensor operation), such as \texttt{matrixMultiply}, \texttt{matrixAdd}, \texttt{relu}, \texttt{softmax}, \texttt{2DConvolution}, etc.

A model inference function which is opaque in the top-level IR could be lowered to the second-level IR for analysis and co-optimization with the relational query processing.

Then all computations will be further lowered to LLVM IR for code generation, as illustrated in Fig.~\ref{fig:mlir}.

\begin{figure}[H]
\centering{%
   \includegraphics[width=3.4in]{Figures/mlir.pdf}  
}
\caption{\label{fig:mlir} Illustration of the multi-level intermediate representation
}
\end{figure}


==> kernel.tex <==
\section{Kernel-Level Comparison}
\label{sec:ffnn}
\subsection{Dense Layer}
\subsubsection{Relation-Centric Representation}
As illustrated in Fig.~\ref{fig:ffnn}, a dense layer consists of a matrix multiplication, a matrix addition, and an activation. As discussed and demonstrated in our previous works~\cite{jankov2019declarative, yuan2020tensor}, in RDBMS, a matrix multiplication can be computed as a \texttt{join} query followed by an \texttt{aggregate} query. A matrix addition can be computed as a \texttt{join}. An activation can be computed as a \texttt{selection}. 

\subsubsection{UDF-Centric Representation} All computations, such as matrix multiplication, matrix addition, and activation, are encapsulated in one user defined function. A \texttt{transform} operator will apply the function to each feature vector in the input set.

\subsubsection{Evaluation Methodology} We first determine a range of the depth (e.g., number of layers) and width (e.g., number of neurons at each layer) of dense layers  in different real-world workloads, including DLRM, DeepSpeech, BERT, VGG$16$, ResNet, and other small scale models that we found in Kaggle. Then, we compare various representations in netsDB, as well as our implementations in TensorFlow and PyTorch with CPU and GPU. 

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:ffnn-overall-1} {\small \color{black} Size of FFNN/MLP in popular models}}
\begin{tabular}{|l|l|l|} \hline
model type& FC type &Shape\\\hline \hline
DLRM-RMC3&DenseFC&$2,560\times128\times32$\\ \hline
VGG-19&FC&$4,096\times4,096\times1,000$\\\hline
keras-BERT&EncoderFC&$768\times3,072\times768$\\\hline
MLP-mixer-Huge&channel-mixing FC&$1,280\times5,120\times1,280$\\ \hline
Amazon-14k&FC&$597,540\times1,024\times14,588$\\ \hline
\end{tabular}
\end{table}

\subsubsection{Results}
The results are illustrated in Tab.~\ref{fc-results}. 

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{fc-results} {\small \color{black} Representations for Fully Connected Layers (FC) in one AWS r4xlarge instance (Unit:Seconds) }}
\begin{tabular}{|p{1.5cm}|p{0.4cm}|p{0.6cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|} \hline
FC-type&UDF&Relation&PyTorch1&PyTorch2&TF1&TF2\\\hline \hline
DLRM-RMC3/DenseFC&$\textbf{3.2}$&$55$&0.00717568397521972&NA&0.2023143768310547&NA\\ \hline
VGG-19/FC&$\textbf{12.8}$&$56$&0.3096446990966797&NA&Time: 0.8139679431915283&NA\\\hline
keras-BERT/EncoderFC&$\textbf{4.2}$&$55$&0.07796335220336914&NA&0.32042765617370605&NA\\\hline
MLP-mixer-Huge-channel-mixing&$\textbf{6.2}$&$37$&0.20032811164855957&NA&0.5937259197235107&NA\\ \hline
Amazon-14k&Failed&$\textbf{208}$&93.10449385643005&79.17961287498474&121.75439691543579&52.12351107597351\\ \hline
\end{tabular}
\vspace{-10pt}
\end{table}

\subsection{Convolutional Layer}
\subsubsection{Relation-Centric Representation}
As illustrated in Fig. 2, a
convolutional layer operation involves computing a set of Hadamard products. As shown in [reference to memfusion paper] this operation can be converted to a large matrix multiplication operation. In the relation-centric approach, this large matrix is stored as a set of matrix blocks, and multiplication is performed on the matrix blocks using a \texttt{join} followed by an \texttt{aggregate}.
\subsubsection{UDF-Centric Representation}
The convolution operation using Eigen spatial convolution or call to a library method such as Aten (Pytorch) can be encapsulated in one user defined function. 

\subsubsection{Evaluation Methodology}
We took widely used models considered in DeepBench CNN inference benchmark [reference to github?]. Then, we compare various representations in netsDB, as well as our implementations in TensorFlow and PyTorch with CPU and GPU.

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:ffnn-overall-1} {\small \color{black} Size of CNN in popular models}}
\begin{tabular}{|l|l|l|} \hline
model type & Image/Input Shape & Kernel Shape \\\hline \hline
DeepBench-CONV1&$112\times112\times64$&$64\times64\times1\times1$\\ \hline
DeepBench-CONV2&$56\times56\times256$&$128\times256\times1\times1$\\ \hline
DeepBench-CONV3&$7\times7\times512$&$2048\times512\times1\times1$\\ \hline
DeepBench-CONV4&$341\times79\times32\times4$&$32\times32\times5\times10$\\ \hline
RetinaMNIST-DeepBench-CONV3&$1\times1736\times1824\times3$&$2048\times3\times1\times1$\\ \hline
LandCover-DeepBench-CONV3&$1\times2500\times2500\times3$&$2048\times3\times1\times1$\\ \hline
\end{tabular}
\end{table}

\subsubsection{Results}
The results are illustrated in Tab.~\ref{fc-results}. 

\begin{table*}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{fc-results} {\small \color{black} Representations for Convolution (CNN) in one AWS r4xlarge instance (Unit:Seconds) }}
\begin{tabular}{|p{2cm}|p{0.7cm}|p{0.7cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|} \hline
CNN-type&UDF&Relation&PyTorch1&TF1&PyTorch2&TF2\\\hline \hline
DeepBench-Conv1&$\textbf{3.6}$&$30$&$0.06283235549926758$&$0.40276312828063965$7&$0.21681976318359375$&$0.40506482124328613$\\ \hline
DeepBench-Conv2&$\textbf{3.6}$&$30$&$0.06395268440246582$&$0.47894835472106934$&$0.23807740211486816$&$0.46279430389404297$\\ \hline
DeepBench-Conv3&$\textbf{3.7}$&$35$&$0.034270286560058594$&$0.45046567916870117$&$0.2265784740447998$&$0.46639227867126465$\\ \hline
DeepBench-Conv4&$\textbf{3.6}$&$41$&$0.23665285110473633$&$0.6699254512786865$&$0.36020445823669434$&$0.6165115833282471$\\ \hline
RetinaMNIST-DeepBench-CONV3&Fail&64&Fail&Fail&Fail&Fail\\ \hline
LandCover-DeepBench-CONV3&Fail&459&Fail&Fail&Fail&Fail\\ \hline
\end{tabular}
\vspace{-10pt}
\end{table*}

\subsection{Word2Vec Layer}
As illustrated in Fig.~\ref{fig:word2vec}, there are two approaches to implement a lookup of embedding vectors for a sequence of $k$ words (or tokens). First, we can implement it as a matrix multiplication between the concatenation of $k$ one-hot vectors that represent the sequence of tokens, and the embedding matrix. Second, if the embedding matrix supports indexing, we can lookup the embedding vector simply based on each sparse ID represents a token in the sequence, and then sum up the output embedding vectors. The latter approach is also known as the implemented  as  the SparseLengthsSum operator in PyTorch~\cite{pytorch}.

\subsubsection{Relation-Centric Representation}
In the relation-centric representation, a matrix is stored as a set of matrix blocks. The first implementation based on matrix multiplication can be represented as a \texttt{join} followed by an \texttt{aggregate}. The second implementation based on index lookup can be represented as a \texttt{select} with the filtering predicate being the equality check on the row index of each embedding vector. We further implement a hash index to accelerate the filtering.  

\subsubsection{UDF-Centric Representation} The two implementations can also be encapsulated to the UDFs, which contain a member that stores the embedding matrix. %

\subsubsection{Evaluation Methodology} 
We first determine a range of word2vec embedding layers that are used in real-world models, including DLRM and BERT from MLPerf, as well as popular language processing models that are publicly available from TF-Hub, as illustrated in Tab.~\ref{tab:embedding-overall-1}.  Then, we compare various representations in netsDB, as well as our implementations in TensorFlow and PyTorch with CPU and GPU. 

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:embedding-overall-1} {\small \color{black} Size of Embedding Layer in popular models}}
\begin{tabular}{|l|l|l|l|} \hline
model type& dictionary size &embedding vector&seq length\\\hline \hline
DLRM-RMC1-2&$180\times10^5$&$32$&$80$\\ \hline
MLPerf-BERT&$10^6$&$768$&$384$\\ \hline
TF-Hub-Word2Vec-Wikipedia&$10^6$&$500$&$10-10,000$\\ \hline
keras-BERT&$10^6$&$768$&$10-10,000$\\ \hline
\end{tabular}
\end{table}

\subsubsection{Results}
The results are illustrated in Tab.~\ref{}. 

\subsection{LSTM Layer}




==> methodology.tex <==
\section{Experimental Overview}
\label{sec:methodology}

In order to provide a comprehensive performance study, we design a benchmark that compares different implementations of model inferences at (1) the kernel-level, which implements kernel operations or layers that are important to deep learning workloads, similar to DeepBench~\cite{deepBench}; (2) the model-level, which implements end-to-end model inference process, similar to MLPerf~\cite{MLCommons}; and (3) the database application level, which nest the database queries from TPC-H, TPC-DS and TPC-C with model inferences.

\subsection{Comparison of Kernel Operations}
\subsubsection{Dense (Fully-connected) Layer}
 As illustrated in Fig.~\ref{fig:ffnn}, at a dense layer, the weight tensor is multiplied with the input feature vector (or a tensor that represents a batch of inputs). The output is then added with the bias vector. The output tensor is applied with an activation function ($\sigma$), such as \texttt{relu} and \texttt{sigmod}. Then the final output is sent to the next layer, which will be computed similarly.

\begin{figure}[h]
\centering
\vspace{-10pt}
\includegraphics[width=0.4\textwidth]{Figures/ffnn.pdf}
\caption{\label{fig:ffnn} \small
Illustration of Dense (Fully-Connected) Layers
}
\end{figure}

\subsubsection{Convolutional Layer}

As illustrated in Fig.~\ref{fig:cnn}, at a convolutional layer, a filter shifts across the input feature tensor. At each shifting step, the filter is mapped to a restricted area in the input tensor, called as a receptive field, then the sum of all elements of a Hadamard product of the receptive field and the filter is computed and added to a bias value. The result becomes a value in the corresponding position of an output feature map.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/cnn.pdf}
\caption{\label{fig:cnn} \small
Illustration of the Convolutional Layer
}
\end{figure}

\subsubsection{Word2Vec Embedding}
\label{sec:word2vec}
A word2vec embedding layer maps a word in a dictionary to an embedding vector. Usually, it is stored as an $n\times d$ matrix, where $n$ represents the size of the dictionary, and $d$ represents the dimension size of a word embedding vector, as illustrated in Fig.~\ref{fig:word2vec}. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/word2vec.pdf}
\caption{\label{fig:word2vec} \small
Illustration of the Word2Vec Embedding Layer
}
\end{figure}

\subsubsection{Long Short-Term Memory}
While afore-mentioned DNN models only accept fixed-size vectors as inputs, Recurrent Neural Network (RNN), such as LSTM, can combine the input vector with their state vector to produce a new state vector that will be combined with the next input vector. This makes it popular and powerful in processing sequence/time-series data. %
As illustrated in Fig.~\ref{fig:lstm}, for LSTM, at each time step $t$, an event ($x_t$) is sent to the LSTM unit, as well as the long-term memory (also called as the cell state $C_{t-1}$) and the short-term memory (also called as the hidden state $h_{t-1}$) obtained from last time step $t-1$. Running computations as illustrated in Fig.~\ref{fig:lstm}, the LSTM unit outputs the updated long-term memory ($C_{t}$) and short-term memory ($h_{t}$) for processing the next event $x_{t+1}$. At the same time, it outputs $o_t$ as the output at time step $t$. If there exists a downstreaming layer of LSTM unit, the $o_t$ and $h_t$ will be  passed to the next layer.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{Figures/lstm.pdf}
\caption{\label{fig:lstm} \small
Illustration of an LSTM Unit
}
\end{figure}


\subsection{Comparison of Full DNN Models}
Now we mainly consider the inference latency of full DNN models in three scenarios, where the features are usually extracted from datasets stored in relational databases. Among the models, the DLRM model is from the MLPerf benchmark and other models are found in public ML community such as Kaggle. 

\subsubsection{Personalized Recommendation}

We consider two types of recommendation tasks. 

The first task infers whether a customer will purchase a product, which is a binary classification problem, based on features extracted from transaction records. We mainly utilize the DLRM model~\cite{} proposed by Facebook for this task. In the DLRM model, categorical features are processed using embeddings, while continuous features are processed with a bottom multilayer perceptron (MLP). Then, second-order interactions of different features are computed using a factorization machine. Finally, the results are processed by a top MLP and fed into a sigmoid function in order to give a probability of a product. We generate model parameters randomly at different scales for performance comparison.

The second task infers a set of products a customer will purchase, which is a multi-label classification problem, also based on features extracted from transaction records. We utilize a FFNN for the Amazon 14K extreme classification task. This model consists of the two layers. The input includes $1,000$ data points that have $597,540$ features, and the extreme classification task uses $14,588$ labels. The hidden layer has $1,000$ neurons.


\subsubsection{Time Series Forecasting}
Deep learning is more and more used for time-series forecasting, which has a significant number of applications over RDBMS, such as predicting retail trade, predicting stock price, and predicting product price, etc. Usually there are following deep learning models widely used for time series forecasting: CNN, LSTM, and CNN-LSTM. We propose three benchmark tasks correspondingly, which are found from Kaggle~\cite{}.

The first task is a CNN model that consists of a Conv1D layer using $64$ filters of size $2$, a max pooling layer of size $2$, a flatten layer, a Dense layer with $50$ neurons and relu activation and an output layer with a sigmoid function.

The second task uses a layer of $50$ LSTM units followed by an output dense layer with a sigmoid function.

The third task combines the aforementioned CNN model and the LSTM model sequentially.

\subsubsection{Credit Card Fraud Detection}
FFNN, CNN, and LSTM are often used for detecting credit card fraud transactions. We proposed three benchmark tasks correspondingly, which are found in a popular Kaggle competition~\cite{}.

The first task used a layer of $20$ LSTM units followed by a top dense layer and then a sigmoid function.

The second task used a FFNN that consists of five dense layers, with each layer having $32$, $16$, $8$, $4$, $1$ neurons respectively.

The third task used two CNN units followed by a dense layer. Each CNN unit consists of a Conv1D layer, a batch normalization layer, and a drop out layer.

\subsubsection{Text classification}
Each model uses three layers. The first layer is a Word2Vec layer  as mentioned in Sec.~\ref{sec:word2vec}, using a vocabulary size of one million and an embedding dimension of $500$. The second layer is a fully connected layer that consists of merely $500\times16$ parameters, and the third layer is an output layer that consists of $16\times2$ parameters.



\eat{\subsubsection{Feed-forward Neural Network}






















}

\subsection{Comparison of SQL Queries nested with Model Inferences}

We selected seven use cases from TPCx-AI and modified these use cases to focus on deep learning models and an end-to-end model serving scenario that includes data cleansing, feature extraction, and model inference. The modified use cases are:

\vspace{5pt}
\noindent
(1) Sales Forecasting. It predicts weekly sales for each store given a limited history of sales data. 
The features are extracted from four tables: orders, product, lineitem, and store\_department. 
We used the LSTM model for this use case. 
The targeting scenario nests three sub queries. The first sub query extract the features, the second sub query runs the LSTM model to make inference on the features, and the third sub query select all stores whose forecasted sales is above $1$ million dollars.

\vspace{5pt}
\noindent
(2) Spam Detection. It detects spam content given a set of input comments, reviews, or descriptions in the context of a retail setting. 
A text classification model is used for this use case, which consists of a word2vec embedding followed by an FFNN.
The targeting scenario also nests three sub queries for feature extraction, model inference, and counting the detected spam contents respectively.

\vspace{5pt}
\noindent
(3) Price Prediction.  It predicts a price of a retail item
based on its brand, product name, and description on an online marketplace, all of which are extracted from the database. 
We used the LSTM model for this use case. 
The query will first extract features and make inferences for each retail item, and then it returns the items whose price changes (the gap between the predicted price and most current price) are higher than a threshold.


\vspace{5pt}
\noindent
(4) Hardware Failure. It predicts impeding failures of hardware based on data and logs collected for every drive. 
The features are extracted from logs of hardware events pre-aggregated per day, containing components IDs, date, and events. 
We used a FFNN model and an LSTM model for this use case.
The nested three sub queries are for feature extraction, model inference, and counting the components that are predicted with failures, respectively.

\vspace{5pt}
\noindent
(5) Product Rating. It emulates a recommender system in the online retail environment. 
The features are extracted from the shopping history of the customers as well as their ratings of historically purchased products.
We used the DLRM model in this case.
The benchmark query will extract features for each customer and recommends products for each customer.

\vspace{5pt}
\noindent
(6) Classification of Customer Shopping Trips. It predicts the type of each shopping trip, such as weekly grocery shopping trip, Christmas shopping trip, etc, based on the items bought in the trip. 
The benchmark query will extract features for each transaction, make inference for each transaction, and return the shopping trip type that are associated with the most transactions.
We test the query using an FFNN model and a CNN model respectively.

\vspace{5pt}
\noindent
(7) Fraud Detection. It evaluates whether a financial transaction is fraudulent or not based on features such as relative amount of the transaction, and the transaction time, which are extracted from historical transaction logs.
The benchmark query will extract features for each transaction, make inference for each transaction, and return the total number of transactions that are detected as fraud.
The query is tested using an FFNN model, an LSTM model, and a CNN model respectively.

Now we explain why we didn't choose the other three use cases of TPCx-AI benchmark. We didn't consider the customer segmentation use case, mainly because it is less common to apply deep learning algorithms to such clustering problem. We didn't select the customer conversion transcription case and the facial recognition case because in these two scenarios, the audio data and image data are not stored in the database, and only the paths to the audio files and image files are stored in the database. So in these scenarios, features are not solely extracted from the database.  We will investigate such workloads in our future works, and in this paper we will focus on scenarios where all features are extracted from the database.

\eat{
We first create four representative queries that nest with full DNN models in aforementioned scenarios, as illustrated in Fig.~\ref{fig:inference-queries}.
The first query recommends product to a customer after a transaction by the customer. The second query predicts the number of airline passengers for different time periods in the next three days, based on airline passenger information in the last sixty days. The third query select all information regarding transactions that are made today and detected as fraud with confidence larger than $85\%$. The fourth query returns the total number of frames collected today, from each of which at least one traffic rule violation is detected.

\begin{figure}[h]
\centering
\vspace{-10pt}
\includegraphics[width=0.4\textwidth]{Figures/inference-queries.pdf}
\caption{\label{fig:inference-queries} \small
Illustration of Nested Relational and DNN Processing
}
\end{figure}

We also modified TPC-H and TPC-C queries to nest with inferences on price, supplier cost, sales, shipping date, and fraud order detection, as illustrated in Fig.~\ref{}.}





\subsection{Platforms Considered}
\subsubsection{netsDB}

\subsubsection{TensorFlow}

\subsubsection{PyTorch}

\subsection{Experimental Environments}


==> model.tex <==
\section{Model-Level Comparison}
\label{sec:cnn}


==> nested-queries.tex <==
\section{Comparison for Queries Nested with Model Inferences}
\label{nested-sql}


==> optimization.tex <==
\section{Query Optimization}
Given an inference query that is represented in such two-level IR, we can further optimize the query execution plan by rewriting the IR for generating more efficient code. We identified several challenges that an inference query optimizer should address.

\vspace{5pt}
\noindent
\textbf{Challenge 5.} How to tune the granularity of UDFs and balance the UDF-centric and relation-centric representations for executing the same type of queries?
\textcolor{red}{Hong: Question: Since relational centric approach is more general fine-grained operations when compared to UDF,  do you see the set of relational-centric operators as something that can grow over time and replace UDF in common  situation? An analogy in hardware is that  relation-centric is like general purpose CPU instructions while UDF is like FPGA for custom functions  } 

For each linear algebra kernel, it can be executed as a combination of relational operators, which is called as relation-centric representation, as illustrated in Fig.~\ref{}. At the same time, one or more linear algebra kernel can be encapsulated into a UDF and from the UDF we may invoke APIs from high-performance linear algebra libraries to perform the computation, as illustrated in Fig.~\ref{}. As shown in Tab.~\ref{fc-results} and Tab.~\ref{cnn-results}, each representation has its limitations. The relation-centric representation works well for large-scale tensors that exceed available memory, but it incurs significant overheads for processing small tensors. On the contrary, the UDF-centric representation can leverage existing advances in linear algebra optimization and GPU acceleration, but it requires all tensors involved fit to memory. (If the size of the tensor is too small, moving the tensor from CPU to GPU could become a bottleneck, because the inference process may not enjoy much benefits from GPU acceleration, which we will discuss in Sec.~\ref{sec:codegen}.)
It is truly a complex optimization problem in determining which linear algebra kernel(s) should be encapsulated as UDFs and which should be broken down to relational operators.

However, there also exists an opportunity that the shape of each model parameter tensor is known since the model is loaded into the RDBMS. Utilizing this opportunity, we may maintain a dynamic tensor size threshold by tracking the available memory size in the hosts and GPU devices. 

We then analyze the proposed two-level IR to dynamically encapsulate linear algebra kernels into UDFs using the following steps: %
\textbf{Step 1.} Assign each edge with a weight that represents the size of the tensor associated with the edge. 
\textbf{Step 2.} Find the maximum induced subgraph satisfying that (1) it has one or more ingress edges but only one egress edge, (2) the weight of each edge in the subgraph is below the pre-specified threshold. This subgraph will be abstracted as \texttt{transform} that is customized by
a UDF that encapsulates the logic for transforming source tensors of this subgraph to the output tensor. Then, the subgraph will be assigned UDF name, which is represented as an opaque node in the top-level IR. 
\textbf{Step 3.} Repeat Step 2, until it cannot find any qualified subgraph.
\textbf{Step 4.} In the resulting graph, each vertex should have at least one ingress edge that has a weight no smaller than the threshold. Such vertex will be expanded into relational operators following the tensor relational algebra~\cite{DBLP:journals/pvldb/YuanJZTBJ21}.

\vspace{5pt}
\noindent
\textbf{Challenge 6.} How to perform accuracy-aware query optimization?

Different with traditional database query optimization that is focusing on computational costs and I/O costs, the inference query execution may benefit from model compression (e.g., quantization, pruning, knowledge distillation, etc.)~\cite{}, which may affect the accuracy of model inference. Such model compression techniques replace the model using a smaller and less accurate model to strike a trade-off between latency and accuracy. While this is a popular optimization technique for model serving, the research question is how to incorporate such technique into the RDBMS query optimization framework. 

A potential approach is to implement various model compression techniques as pre-defined approximate transformations (versus equivalent transformation in traditional query optimization), which rewrites the IRs by modifying the model inference logic to use less amount of parameters.  \textcolor{red}{Hong: Question: Is the optimization problem itself a complex problem (NP-hard?)  will heuristics-based approach be sufficient?  I guess it depends on if the inaccuracy  gets magnified with multiple relation-centic steps in the pipeline?   } 

Another approach is to leverage existing works in AutoML for model compression~\cite{} to explore a vast search space of compressed model architectures, and evaluate the latency and accuracy along the searching process. 




\vspace{5pt}
\noindent
\textbf{Challenge 7.} How to enhance the RDBMS physical optimization process to integrate with today's popular model serving techniques? 

In addition to model compression, there are many other popular optimization techniques widely applied to today's model serving platforms~\cite{}. These techniques include but are not limited to caching of inference results~\cite{}, dynamic batching~\cite{}, prefix batching~\cite{}, etc. We identified the following opportunities.

\noindent
\textbf{Indexing Inference Results for Caching.} We investigated leveraging database indexing to serve as a inference result cache. The idea is to create a table to record the features of frequent inference requests as well as the prediction results. We then apply indexing to the feature fields to facilitate query of prediction results from the table. %

\noindent
\textbf{Vectorized UDF for Dynamic Batching.} Each deep learning operation (e.g., a kernel) may desire a different batch size in a given system~\cite{}. We propose to generate vectorized code for UDFs and relational operators, so that each operator takes one batch of inference samples at a time. We also need to modify the vectorization logic, so that each operator can use a different batch size and the batch size could change over time based on the variability of the available system resources.

\noindent
\textbf{Storage and Computation Sharing for Prefix Batching.} Prefix batching is a model serving optimization technique that shares the batching of inference requests across models that have a lot of the layers in common while each model specializes only a few layers. One common example of such scenario is to serve multiple models that are obtained through transfer learning from one foundation model. 
One approach to facilitate storage sharing is to leverage our previous works in model deduplication to ensure that a tensor that is shared by many models will have only one copy on disk and in memory. 
In addition to the storage sharing, a more challenging problem is how to share computation across different inference queries. To make the shared computation related to the same tensor visible to multiple queries, we need to adopt a multiple-query physical optimization approach~\cite{}. We believe it will lead to numerous research questions.










==> runtime.tex <==
\section{Inference Query Execution Runtime}
\label{sec:runtime}

In order to support the high-performance execution of inference queries, the traditional database runtime is faced with new challenges as described below:

\vspace{5pt}
\noindent
\textbf{Challenge 7.} UDFs may invoke APIs from external linear algebra libraries, where the threading may be managed separately (e.g., by OpenMP), so how to perform unified resource scheduling? 

In order to coordinate the resources between the database runtime and the external libraries, it is important to correctly configure the hyperparameters, such as the number of threads for the database query processing, and for OpenMP, as well as the sizes of memory buffers. Recent works in AI-enhanced databases~\cite{butrovich2022tastes, ma2018query, zhou2020database, zhang2019end}, propose to leverage AI/ML models to automatically tune the hyperparameters, which may create an opportunity for addressing the unified resource management challenge. %



==> serving.tex <==

The RDBMS has to support popular model serving techniques, which could be a significant challenge.

\noindent
\textbf{Challenge 8.} How to enhance the RDBMS to integrate today's popular model serving techniques? 

There are many other popular optimization techniques widely applied to today's model serving platforms~\cite{crankshaw2017clipper, shen2019nexus, olston2017tensorflow, yi2018factorized, lee2018pretzel}. These techniques include but are not limited to the caching of inference results~\cite{crankshaw2017clipper, balasubramanian2021accelerating, kumar2019accelerating}, dynamic batching~\cite{ali2020batch, shen2019nexus}, partitioning models and packing model partitioning to GPU devices\cite{shen2019nexus}, etc. We identified the opportunities for each technique.

\noindent
\textbf{Caching of Inference Results.} One option is to leverage database indexing to serve as an inference result cache. The idea is to create a table to record the features of frequent inference requests as well as the corresponding prediction results. We then construct nearest neighbor indexing over the features to facilitate inference queries. 

This idea overlaps with recently emerging vector databases, such as Pinecone~\cite{pinecone}, Milvus~\cite{milvus}, Faiss~\cite{faiss}, Qdrant~\cite{qdrant}, Vespa~\cite{vespa}, which store vectors such as embedding vectors used in language models, and  build various indexing to facilitate nearest neighbor search, including hierarchical navigable small world (HNSW)~\cite{malkov2018efficient}, locality sensitive hashing (LSH)~\cite{zhu2016lsh}, inverted file indexing (IVF)~\cite{sivic2003video}, and product quantization~\cite{jegou2010product}.  How to integrate those systems/functionalities into RDBMS to facilitate the caching of inference results and accelerate fast inference results without running the inference computations could be an interesting research question. %

\noindent
\textbf{Dynamic Batching.} Batching could balance the latency, throughput, and resource utilization. Each deep learning operation (e.g., a kernel) may desire a different batch size in a given system~\cite{shen2019nexus, ali2020batch}. One option is to leverage the vectorized data processing operator and database pipelines (i.e., each database pipeline is a series of fused data processing operators). However, the vectorization and pipelining logic should be enhanced, so that each operator can use a different batch size and the batch size could change over time based on the variability of the available system resources.

\noindent
\textbf{Partitioning Models and Packing Model Partitions to Different  Devices for Serving.} The scheduling of database pipeline stages in traditional OLAP database is mostly  using a bulk synchronous parallel (BSP) model. Each pipeline stage is executed using many threads. All threads run the same processing logic on different input splits~\cite{shi2014mrtuner}. The assumption is that there are a large number of input splits, but the processing of each set of concurrent input splits fits the available resources~\cite{shi2014mrtuner}. %
For inference queries, an operator may be applying a large-scale model to an input split. There are two options to solve the problem: (1) When the model fits memory, we can tune the input split size for the BSP model. (2) When the model doesn't fit memory, it is important to adapt the BSP model to model partitioning, where a large model is partitioned into layers, and each layer runs on a different device, which is similar to the pipeline parallelism concept in model training~\cite{huang2019gpipe, narayanan2019pipedream}.  One potential solution is to partition the operators in one database pipeline stage to multiple available devices. %

In addition, resource management frameworks for multi-tenant analytics databases, such as Yarn~\cite{vavilapalli2013apache} and Mesos~\cite{hindman2011mesos}, allow the sharing of system resources for the running of multiple workloads at the same time. Such frameworks may be leveraged for packing the inference queries that involve small models.



==> storage.tex <==
\vspace{-10pt}
\section{Storage and Memory Management}
\label{sec:storage}

Tensor data (e.g., the weight matrices in deep learning models), and vector data (e.g., features and embedding vectors), are not relational in nature. 
However, the inference queries need to manipulate both relational data and tensor/vector data.Therefore, the RDBMS is faced with a storage challenge as follows.



\vspace{5pt}
\noindent
\textbf{Challenge 9.} How to manage the storage and caching of relational data, tensor data, and vector data in a unified way? 

One straightforward solution, as adopted in many Big Data analytics frameworks, is to convert tensor/vector data into relation by blocking each tensor/vector as a collection of tensor/vector blocks. Each collection is similar to a relation that has attributes such as \texttt{block\_row\_Id}, \texttt{block\_column\_id}, and  \texttt{block\_data}~\cite{meng2016mllib, boehm2016systemml}. However, the problem is more complicated. First, the query optimizer needs to distinguish model data from other types of data, in order to facilitate accuracy-aware query optimization and ahead-of-time query compilation.  For example, the fuzziness of relational data and tensor/vector data is different. While relational data must be stored exactly, some errors/approximations in the tensor/vector data may not significantly affect the application accuracy. Second, different from normal data, tensor/vector data may introduce a significant amount of redundancy and sparsity, which can be further leveraged for deduplication and compression in order to reduce storage costs and memory footprint~\cite{DBLP:journals/pvldb/ZhouCDMYZZ22, schleich2023optimizing}. Third, the indexing of normal data and tensor/vector data have different structures. The latter uses approximate indexing more than exact indexing. Therefore, it is important to enhance the database catalog to specify the metadata information such as how a tensor relation is shared in different models in order to facilitate query optimization, compilation, model deduplication, and approximate indexing for similarity-based search. In addition, as discussed in Challenge 2 (Sec.~\ref{sec:optimization}), it is important to investigate the automatic tiling  of the tensors and distributing of the tensor blocks to accelerate the inference task~\cite{luo2021automatic,zou2021lachesis} as part of the physical database design~\cite{agrawal2000automated, rao2002automating}.


==> summary.tex <==
\section{Summary of Findings}
\label{sec:summary}


==> transaction.tex <==
\section{Integrated Transaction and Analytics Processing}
\label{sec:transaction}

The inference query may be mixed with transaction processing. As illustrated in Listing~\ref{lst:transaction}, the application logic  is greatly simplified by integrating the fraud detection of a credit-card transaction into a transaction, so that the accounts' balances will only be updated if the transaction is authentic. 

\vspace{-10pt}

\begin{lstlisting}[
        caption={An example transaction mixing model inferences},label={lst:transaction},
           language=SQL,
           showspaces=false,
           basicstyle=\ttfamily\footnotesize,
           numbers=left,
           numberstyle=\tiny,
           commentstyle=\color{gray},
           breaklines=true
        ]
BEGIN;
INSERT INTO transactions VALUES ($transaction_id, $processor_id, $processor_name, $transaction_type, $document_no, $document_type, $document_group, $customer_id, $currency_id, $account_no, $amount, $auth_code, $card_type, $created_on);
UPDATE transaction_fraud_detection SET fraud = (SELECT (fraud_dnn.predict(*))FROM transactions WHERE transaction_id=$transaction_id) WHERE transaction_id=$transaction_id;
UPDATE accounts SET balance = balance - $amount WHERE account_no = $account_no_to_debit AND (SELECT fraud FROM transaction_fraud_detection WHERE transaction_id=$transaction_id)=False;
UPDATE accounts SET balance = balance + $amount WHERE account_no = $account_no_to_credit WHERE account_no = $account_no_to_debit AND (SELECT fraud FROM transaction_fraud_detection WHERE transaction_id=$transaction_id)=False;
COMMIT;

\end{lstlisting}

It is important to keep up the credit card transaction throughput and ensure it will not be bottlenecked by the model inference computation. Despite that there exist many challenges that have been discussed in hybrid transaction and analytics processing (HTAP) ~\cite{huang2020tidb, lee2017parallel, makreshanski2017batchdb, mozafari2017snappydata, barber2016wildfire}, due to limited space, we focus on the following challenge related to batching:

\vspace{5pt}
\noindent
\textbf{Challenge 10.} How to schedule transactions that involve inference queries with dynamic batching to maximize resource utilization and concurrency?

Model inference computations, depending on the models,  could be significantly more computational-intensive than traditional transaction operations.  In addition, the DL model can better utilize system resources through the batching of inference computations, which may provide new opportunities for transaction batching~\cite{ding2015centiman, faleiro2014lazy, choi2021lazy, lu2021epoch}. For example, %
we may consider a look-ahead mechanism that buffers transaction requests, and extracts and groups the inference computations from those requests by models, and executes those  batches ahead of processing the other operations from corresponding transactions. This idea amounts to implementing a new fine-grained locking system with dynamic batching for transactions that involve inferences.











==> vision.tex <==
\eat{

\vspace{-5pt}
\section{Gap Identification and Vision }
\label{sec:vision}

\noindent
\textbf{Performance Gap Identification.} 
None of the existing pivotal architectures perform optimally across all scenarios.  %


Regarding \textbf{latency}, the DL-Centric architecture incurs additional latency for transferring data from/to the RDBMS. For example: \textit{a Tier 1 bank in the US running its core system on an IBM zSystems platform has deployed an off-platform AI-based fraud detection system. Due to latency issues, the bank runs only very high-risk transactions through the AI system. Most transactions are run through rules-based scoring with lower accuracy~\cite{fraud-ibm}.} As illustrated in Fig.~\ref{fig:normalized-breakdown} and Tab~\ref{tab:overall-latency}, for workloads with simple models such as small convolutional networks (e.g., DeepBench-Conv1), or large size of inference data (e.g., Amazon-14K-FC requires $594,540$ features), the data transfer overheads dominate. Conversely, the Relation-Centric and UDF-Centric architectures eliminate such data transfer. However, their inference latency for complex models could be worse than the DL-Centric counterpart. In Table~\ref{tab:overall-latency}, if we deduct the data transfer latency, as illustrated in Fig.~\ref{fig:normalized-breakdown}, from the end-to-end latency for DL-Centric platforms, the DL-Centric platforms outperform UDF-Centric and Relation-Centric in most of the cases except those Out-of-Memory (OOM) cases. One reason is that RDBMS lacks the serving techniques, as discussed in Sec.~\ref{sec:serving}. %

\vspace{5pt}
In terms of \textbf{scalability}, the linear algebra computations in the Relation-Centric architecture can effortlessly scale up to accommodate massive tensors that exceed memory limitations. This capability stems from its ability to split a single tensor into blocks and spill partial tensor blocks to disk, leveraging the RDBMS buffer pool management. In contrast, most of today's DL runtimes and libraries encounter out-of-memory (OOM) errors in such situations, as illustrated in Tab.~\ref{tab:overall-latency}. That's because these libraries consider a tensor to be the smallest unit of objects and there is no data management layer to split a tensor into blocks and run tensor operations on top of a collection of blocks with only a portion of the blocks residing in memory and the rest of blocks in memory.

\begin{table}[h]
    \centering
    \scriptsize
    \caption{\label{tab:ffnn-overall-1}\small Fully Connected (FC) Models (one hidden layer)}
    \begin{tabular}{cc}
        \toprule
        Model & Number of Features/Number of Neurons (hidden layer size)/Outputs \\
        \midrule
        Keras-Bert-Encoder-FC&$76/3,072/768$ \\
        Amazon-14k-FC&$597,540/1,024/14,588$ \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \scriptsize
    \caption{\label{tab:cnn-overall-1}\small Convolutional Models}
    \begin{tabular}{ccc}
        \toprule
        Model & Image/Input Shape & Kernel Shape \\
        \midrule
        DeepBench-CONV1&$112\times112\times64$&$64\times64\times1\times1$\\
        LandCover-DeepBench-CONV3&$2500\times2500\times3$&$2048\times3\times1\times1$\\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \scriptsize
    \caption{\label{tab:overall-latency} \small End-to-End Latency Comparison (unit: seconds), UDF-Centric and Relation-Centric representations are implemented on netsDB ~\cite{DBLP:journals/pvldb/ZhouCDMYZZ22}$^{\ref{footnote:netsdb}}$. We compare these to the DL-Centric counterparts using Pytorch-2.0 and TensorFlow-2.0. Experiments were run on an Amazon EC2 r4.2xlarge instance with eight CPU cores and $62$ GB memory. The architecture of these models or kernels can be found in Tab.~\ref{tab:ffnn-overall-1} and Tab.~\ref{tab:cnn-overall-1}. The state-of-the-art ConnectorX~\cite{wang2022connectorx} was used as the Postgres connector.}
    \begin{tabularx}{0.48\textwidth}{@{} c X X X X X @{}}
        \toprule
        Model & Batch Size & Relation-Centric & UDF-Centric & DL-Centric (Postgres+ TF) & DL-Centric (Postgres+ Pytorch) \\
        \midrule
        \multirow{2}*{Keras-BERT-Encoder-FC} &$1000$ &$12.6$ &$0.5$&$\textbf{0.4}$&$\textbf{0.4}$\\
        &$8000$&$13.4$&$\textbf{0.6}$&$1.5$&$1.0$\\
        \midrule
        \multirow{2}*{Amazon-14k-FC} &$1000$&$58.6$&$60.4$&$34.6$&$\textbf{22.6}$\\
        &$8000$&$\textbf{407.2}$&OOM&OOM&OOM\\
        \midrule
        \multirow{5}*{DeepBench-CONV1} &$64$&$8.9$&$\textbf{0.4}$&$2.8$&$2.8$\\
        &$128$&$10.8$&$\textbf{0.8}$&$5.2$&$5.3$\\ 
        &$256$&$14.8$&$\textbf{1.6}$&$10.0$&$10.2$\\ 
        &$512$&$24.4$&$\textbf{3.3}$&$18.9$&$19.4$\\ 
        &$1024$&$42.5$&$\textbf{6.5}$&$38.3$&$38.9$\\
        \midrule
        \multirow{4}*{LandCover-CONV3} 
        &$1$&$36.8$& OOM & $\textbf{9.9}$ & OOM\\ 
        &$2$&$\textbf{45.2}$& OOM & OOM & OOM\\ 
        &$4$&$\textbf{46.6}$& OOM & OOM & OOM\\
        &$8$&$\textbf{49.6}$& OOM & OOM & OOM\\
        &$16$&$\textbf{76.9}$& OOM & OOM & OOM\\
        \bottomrule
    \end{tabularx}
\end{table}

\footnotetext[1]{{\label{footnote:netsdb}NetsDB (https://github.com/asu-cactus/netsdb) is developed on top of PlinyCompute~\cite{zou2018plinycompute,zou2020architecture, zou2020watson, DBLP:journals/pvldb/ZouDBIYJJ21, zou2019pangea}, which is an object-oriented relational database system.}}

\begin{figure}[h]
\centering{%
   \includegraphics[width=3.4in]{Figures/breakdown-vision.pdf}  
}
\caption{\small\label{fig:normalized-breakdown} Breakdown of Normalized Latency of the Model Inference Process into Data Transfer Latency (Blue) and Inference Latency (Green) for different types of DL models. All experiments ran models or kernels from popular models on an Amazon EC2 r4.2xlarge instance with eight CPU cores and $62$ GB memory. The architecture of these models or kernels can be found in Tab.~\ref{tab:ffnn-overall-1} and Tab.~\ref{tab:cnn-overall-1}. The data transfer latency is measured as the latency of reading one batch of data from Postgres using ConnectorX~\cite{wang2022connectorx}. We used Pytorch 2.0 and TensorFlow 2.0. The numbers following the model name indicate the inference data batch sizes.
}
\end{figure}

\noindent
\textbf{Middle Grounds in-between Pivotal Architectures.} We also identified a hybrid representation may achieve significantly better results. Taking Amazon-14k-FC for example, the most memory-intensive operation is the matrix multiplication between the input batch (of shape $batch\_size \times feature\_size$) and the model weight matrix of the first layer (of shape $feature\_size \times hidden\_layer\_size$). 
Other operations are simple and involve significantly smaller tensors. Using Relation-Centric representation for small matrix multiplication or addition will introduce multiple joins, aggregations, and matrix reblocking operations, which are pipeline breakers. Such heterogeneous characteristics among operators motivate a hybrid representation: only apply the Relation-Centric representation to this large-scale matrix multiplication operation, while the rest of the computations are represented in UDF-Centric representation. 

We've found the hybrid representation achieved more than $2.4\times$ speedup compared to the pure Relation-Centric representation and $2.5\times$ speedup compared to the pure UDF-Centric, reducing the latency from $58.6$ seconds to $23.9$, when batch size is $1,000$. (UDF-Centric representation failed when batch size increased to $8,000$.)


 A summary of the specific use scenarios for each of the three pivotal paradigms can be found as follows:

\vspace{5pt}
\noindent\begin{tcolorbox}[enhanced jigsaw,breakable,
title after break=,
left=0mm,right=0mm,bottom=0mm,top=0mm,colback=red!5!white,colframe=red!75!black,
]{

\textbf{$\bullet$ DL-Centric Architecture:} Ideal for scenarios where leveraging unique techniques in DL systems is crucial. It is particularly effective for applications bounded by inference computations with insignificant data transfer overheads. 

\textbf{$\bullet$ UDF-Centric Architecture:} Well-suited for scenarios that require inferences over large batches of data and/or high-dimensional data with relatively simple models. By "simple models," we refer to models that do not require non-compliant serving capabilities within RDBMS (Sec.~\ref{sec:serving}). Additionally, it is essential that each operator in such models can fit into memory.

\textbf{$\bullet$ Relation-Centric Architecture:} Excels in performing large-scale tensor computations with cost constraints, e.g., handling tensors that exceed memory within a single CPU node. In addition, through experiments, we also found that Relation-Centric architecture could outperform UDF-Centric architecture for large-scale matrix multiplications that fit memory because it reduces memory footprint and cache misses by allowing each thread to process a few blocks each time.
}
\end{tcolorbox}

Furthermore, inference applications exhibit diverse natures. As illustrated in Fig.~\ref{fig:normalized-breakdown}, different batch sizes and models lead to divergent inference/data-transfer ratios. In addition, as illustrated in Tab.~\ref{tab:applications}, not only do different applications have disparate characteristics, but also the same application may experience fluctuations in event frequency, necessitating different batch sizes and models at different time points. Given such variability, we advocate for seamlessly integrating these architectures into one cohesive system. %




\begin{table*}[t]
    \centering
    \scriptsize
    \caption{\label{tab:applications} Diverse Requirements of Example Applications}
    \begin{tabular}{lccccl}
        \toprule
        Application & Event Frequency & Desired Latency & DL Models & Batch Size & Functionalities \\
        \midrule
        Customer chatbot~\cite{nvidia-chatbot, chatbots} & 10-10K per sec & <300ms & Jasper, Bert, Tacotron2, etc. & 1-1K & context retrieving, security \& privacy \\

        Fraud detection \& AML~\cite{fraud-ibm, wang2021apan, xilinx-aml} & 1K-1M per sec & <100 ms & LSTM, CNN, GNN, etc. & 100-100K & transaction, security \& privacy, trigger \\

        Recommendation~\cite{ardestani2022supporting, eksombatchai2018pixie, gupta2020deeprecsys} & 1K-100K per sec & <50ms & DLRM, DeepFM, NCF, etc. & 50-5K & security \& privacy \\
        \bottomrule
    \end{tabular}
\end{table*}

\vspace{5pt}
\noindent
 \textbf{Vision: Enabling a Novel Database System.} As shown in Fig.~\ref{fig:representation-overview}d, the novel database connects to DL runtimes, linear algebra libraries, and DNN libraries simultaneously.  It consists of four components: 











\eat{
\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:cnn-overall-1} {\small \color{black} Inference Latency Comparison (unit: seconds)}}
\begin{tabular}{|p{1.5cm}|r|r|r|r|r|} \hline
model type & \#inputs & netsDB-rel & netsDB-UDF & TF & PyTorch \\\hline \hline
\multirow{2}{*}{\parbox{1.5cm}{Keras-BERT-Encoder-FC}}&$1000$&$12.6$&$0.4$&$0.3$&$\textbf{0.1}$\\
&$8000$&$13.4$&$0.6$&$1.2$&$\textbf{0.3}$\\\hline
\multirow{2}{*}{\parbox{1.5cm}{Amazon-14k}}&$1000$&$48.1$&$7.8$&$15.9$&$\textbf{4.7}$\\
&$8000$&$\textbf{407.2}$&failed&failed&failed\\\hline

\multirow{5}{*}{\parbox{1.5cm}{DeepBench-CONV1}
}&$64$&$8.9$&$0.4$&$0.3$&$\textbf{0.2}$\\ 
&$128$&$10.8$&$0.8$&$0.5$&$\textbf{0.3}$\\ 
&$256$&$14.8$&$1.6$&$1.0$&$\textbf{0.7}$\\ 
&$512$&$24.4$&$3.3$&$1.9$&$\textbf{1.3}$\\ 
&$1024$&$42.5$&$6.5$&$3.7$&$\textbf{2.6}$\\ \hline
\multirow{3}{*}{\parbox{1.5cm}{LandCover-CONV3}}&$2$&$\textbf{45.2}$& failed & failed & failed\\ 
&$4$&$\textbf{46.6}$& failed & failed & failed\\
&$8$&$\textbf{49.6}$& failed & failed & failed\\
&$16$&$\textbf{76.9}$& failed & failed & failed\\
\hline
\end{tabular}
\end{table}
}



\eat{\subsection{Fully Connected Layer}
As illustrated in Fig.~\ref{fig:ffnn}, at a dense layer, the weight tensor is multiplied with the input feature vector (or a tensor that represents a batch of inputs). The output is then added with the bias vector. The output tensor is applied with an activation function ($\sigma$), such as \texttt{relu} and \texttt{sigmod}. Then the final output is sent to the next layer, which will be computed similarly.

\begin{figure}[h]
\centering
\vspace{-10pt}
\includegraphics[width=0.4\textwidth]{Figures/ffnn.pdf}
\caption{\label{fig:ffnn} \small
Illustration of Dense (Fully-Connected) Layers
}
\end{figure}

\subsubsection{Relation-Centric Representation}
As illustrated in Fig.~\ref{fig:ffnn}, a dense layer consists of a matrix multiplication, a matrix addition, and an activation. As discussed and demonstrated in our previous works~\cite{jankov2019declarative, yuan2020tensor}, in RDBMS, a matrix multiplication can be computed as a \texttt{join} query followed by an \texttt{aggregate} query. A matrix addition can be computed as a \texttt{join}. An activation can be computed as a \texttt{selection}. 

\subsubsection{UDF-Centric Representation} All computations, such as matrix multiplication, matrix addition, and activation, are encapsulated in one user defined function. A \texttt{transform} operator will apply the function to each feature vector in the input set.

\subsubsection{Evaluation Methodology} We first determine a range of the depth (e.g., number of layers) and width (e.g., number of neurons at each layer) of dense layers  in different real-world workloads, including DLRM, DeepSpeech, BERT, VGG$16$, ResNet, and other small scale models that we found in Kaggle. Then, we compare various representations in netsDB, as well as our implementations in TensorFlow and PyTorch with GPU acceleration. 



\subsubsection{Results}
The results are illustrated in Tab.~\ref{fc-results}. 

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{fc-results} {\small \color{black} Representations for Fully Connected Layers (FC) in one AWS r4xlarge instance (Unit:Seconds) }}
\begin{tabular}{|c|c|c||c|c|} \hline
FC-type&UDF&Relation&PyTorch&TensorFlow\\\hline \hline
DLRM-RMC3/DenseFC&$\textbf{3.2}$&$55$&0.1&0.2\\ \hline
VGG-19/FC&$\textbf{12.8}$&$56$&0.3& 0.8\\\hline
keras-BERT/EncoderFC&$\textbf{4.2}$&$55$&0.1&0.3\\\hline
MLP-mixer-Huge-channel-mixing&$\textbf{6.2}$&$37$&0.2&0.6\\ \hline
Amazon-14k&Failed&$\textbf{208}$&Failed&Failed\\ \hline
\end{tabular}
\vspace{-10pt}
\end{table}

\subsection{Convolutional Layer}

As illustrated in Fig.~\ref{fig:cnn}, at a convolutional layer, a filter shifts across the input feature tensor. At each shifting step, the filter is mapped to a restricted area in the input tensor, called as a receptive field, then the sum of all elements of a Hadamard product of the receptive field and the filter is computed and added to a bias value. The result becomes a value in the corresponding position of an output feature map.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/cnn.pdf}
\caption{\label{fig:cnn} \small
Illustration of the Convolutional Layer
}
\end{figure}

\subsubsection{Relation-Centric Representation}
As illustrated in Fig~\ref{fig:cnn}, a
convolutional layer operation involves computing a set of Hadamard products. As shown in [reference to memfusion paper], this operation can be converted to a large matrix multiplication operation. In the Relation-Centric approach, this large matrix is stored as a set of matrix blocks, and multiplication is performed on the matrix blocks using a \texttt{join} followed by an \texttt{aggregate}.

\subsubsection{UDF-Centric Representation}
The convolution operation using Eigen spatial convolution or call to a library method such as Aten (PyTorch) can be encapsulated in one user defined function. 

\subsubsection{Evaluation Methodology}
We took widely used models considered in DeepBench CNN inference benchmark. Then, we compare various representations in netsDB, as well as our implementations in TensorFlow and PyTorch with GPU acceleration.

\begin{table}[h]
\vspace{-5pt}
\centering
\scriptsize
\caption{\label{tab:cnn-overall-1} {\small \color{black} Size of CNN in popular models}}
\begin{tabular}{|l|l|l|} \hline
model type & Image/Input Shape & Kernel Shape \\\hline \hline
DeepBench-CONV1&$112\times112\times64$&$64\times64\times1\times1$\\ \hline
DeepBench-CONV2&$56\times56\times256$&$128\times256\times1\times1$\\ \hline
DeepBench-CONV3&$7\times7\times512$&$2048\times512\times1\times1$\\ \hline
DeepBench-CONV4&$341\times79\times32\times4$&$32\times32\times5\times10$\\ \hline
RetinaMNIST-DeepBench-CONV3&$1\times1736\times1824\times3$&$2048\times3\times1\times1$\\ \hline
LandCover-DeepBench-CONV3&$1\times2500\times2500\times3$&$2048\times3\times1\times1$\\ \hline
\end{tabular}
\end{table}

\subsubsection{Results}
The results are illustrated in Tab.~\ref{cnn-results}. 

\begin{table}[h]

\centering
\scriptsize
\caption{\label{cnn-results} {\small \color{black} Representations for Convolution (CNN) in one AWS r4xlarge instance (Unit:Seconds) }}
\begin{tabular}{|c|c|c||c|c|} \hline
CNN-type&UDF&Relation&Decoupled-PyTorch&Decoupled-TensorFlow\\\hline \hline
DeepBench-Conv1&$\textbf{3.6}$&$30$&$0.1$&$0.5$\\ \hline
DeepBench-Conv2&$\textbf{3.6}$&$30$&$0.1$&$0.5$\\ \hline
DeepBench-Conv3&$\textbf{3.7}$&$35$&$0.1$&$0.5$\\ \hline
DeepBench-Conv4&$\textbf{3.6}$&$41$&$0.2$&$0.7$\\ \hline
RetinaMNIST-DeepBench-CONV3&Fail&$\textbf{64}$&Fail&Fail\\ \hline
LandCover-DeepBench-CONV3&Fail&$\textbf{459}$&Fail&Fail\\ \hline
\end{tabular}

\end{table}
}






}


==> vision1.tex <==




\eat{

Second, how to incorporate popular model serving techniques such as model compression, caching of inference results, dynamic batching, prefix batching and so on into RDBMS by leveraging and rewriting existing RDBMS functions? We provided several ideas based on indexing, dynamic vectorization, and multi-query optimization to address these challenges.

\vspace{5pt}
\noindent
\textbf{Code Generation.} Inference queries may benefit from GPU acceleration. However, it is challenging to determine which computations should run on GPU devices and how to schedule various computations to fully utilize CPU/GPU resources and to overlap computation and I/O operations. We discussed the possibility of leveraging multi-instance GPU and the producer-transfer-consumer (PTC) model to solve the problems. 

 }

